Fostering new Vertical and Horizontal IoT Applications with Intelligence Everywhere

Intelligence Everywhere is predicated on the seamless integration of IoT networks transporting a vast amount of data streams through many computing resources across an edge-to-cloud continuum, relying on the orchestration of distributed machine learning models. The result is an interconnected and collective intelligent ecosystem where devices, systems, services, and users work together to support IoT applications. This paper discusses the state-of-the-art research and the principles of the Intelligence Everywhere framework for enhancing IoT applications in vertical sectors such as Digital Health, Infrastructure, and Transportation/Mobility in the context of intelligent society (Society 5.0). It also introduces a novel perspective for the development of horizontal IoT applications, capable of running across various IoT networks while fostering collective intelligence across diverse sectors. Finally, this paper provides comprehensive insights into the challenges and opportunities for harnessing collective knowledge from real-time insights, leading to optimised processes and better overall collaboration across different IoT sectors.

==> CONTENTS/Backup_section_IV.tex <==
\section{Future IoT Applications}


vertical and horizontal IoT applications???
most of the iot applications a re vertical,...

+ bring some examples from the IoT use cases
try to link the 3 applications

IoT sensors are another impact factor for designing IoT network infrastructures. Essentially, all the instrumental and smart electronic chips are the segments of sensors that could sense, collect, manipulate, transmit, and analyze data through different analytical workflows. From the perspective of IoT sensors, the pivotal specificities of communication technologies are coverage-range and type. We cannot neglect these two attributes, especially when developing an IoT infrastructure for supporting an analytical workflow. Each communication protocol has a predefined coverage area and every IoT use case has its requirements in terms of the range of communication. 



In this section, we introduce three IoT use cases: wearables, intelligent home, and Internet of Vehicles (IoV). We discuss how their network infrastructure can be integrated into an Analytics Everywhere framework. 

\subsection{Analytics Everywhere for Wearable Applications}
Table \ref{tab:BAN} summarizes the most suitable, stable, and efficient communication technologies available for wearable applications. In a short-range communication scenario (e.g. wireless human sensing, gesture recognition), an RFID solution fits well because of its unique ID. The Wi-Fi based solution is more useful in the non-intrusive type of human sensing due to its wireless characteristics \cite{LiuZWirelessHumanSensing}, a variety of network types (e.g. BAN, WPAN, and WLAN) can be selected, depending on the requirements of a wearable application. Z-wave has a -20 to 0 dBm power ratio and a sleep/awake power saving mechanism, making it an appropriate match for wearable applications from a network management perspective. Since users could manage smart lighting from their smart watches (part of BAN). Z-wave (WPAN) would then give access to a smart hub. Considering energy harvesting and low cost of tags, NFC is crucial for privacy and contactless payments \cite{AntonioNFCsensor}. In terms of coverage range, RF and WirepasMesh can give us the flexibility to go beyond a 100 meter range with IoT wearables. From a security perspective, 6LoWPAN is an exemplary option as it only works with IPv6.

\begin{table*}[!ht]
\centering
\caption{Communication Technologies suited for IoT Wearable Applications.}
\label{tab:BAN}
\resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
\begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
\midrule
ANT & No & Full & WPAN & No & 7.5 - 15 & 1 & \textless 17 & Yes & 30 \\
\begin{tabular}[c]{@{}l@{}}BLE (Bluetooth\\ 4/4.1/4.2/5)\end{tabular} & Yes & Half / Full & BAN / WPAN & Yes & 3, 6 & 1, 2, 3 & 0 -10 & Yes & 15 - 30, 50 - 70, 100 \\
Bluetooth & No & Half / Full & BAN / WPAN & No & 100 & 1 & 0 - 10 & Yes & 1,10,100 \\
EnOcean & Yes & Half & WPAN & No & 40 - 100 & 0.125 & 10 & Yes & 30 \\
Infrared & Yes & Half & WLAN & Yes & 175 & 12500 & 24 & No & 0.001 - 30 \\
NFC & Yes & Half & BAN / WPAN & Yes & 125 & \begin{tabular}[c]{@{}l@{}}0.106, 0.212, \\ 0.424, 0.848\end{tabular} & 20, 23 & No & 0.1 - 0.2 \\
RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
RFID & Yes & Half / Full & WPAN & Yes & 20 & 0.5 & 1.8 & Yes & 0.1 - 5 \\
Thread & Yes & Half & HAN / WPAN & No & 100 & 0.25 & 21 & Yes & 30 \\
Wi-Fi 6 & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & 1.5 & >=1000 & 32 & Yes & 60 - 1000 \\
WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
Zigbee & Yes & Half / Full & WPAN & Yes & 20 & 0.02, 0.04, 0.25 & 20 & Yes & 10 - 100 \\
Z-Wave & Yes & Half & WPAN & No & 3000 & 0.0096, 0.04, 0.1 & -20 - 0 & Yes & 30, 100 \\
6LoWPAN & Yes & Half & WPAN & Yes & 50 - 250 & 0.25 & 3 - 22 & Yes & 10 - 100 \\\bottomrule
\end{tabular}}
\end{table*}

Fig. \ref{fig_BAN-BLE} shows a communication scenario for wearable applications operating in BAN where EoG, ECG, and EMG sensors are attached in the form of a small chipset within wearable devices like a smartwatch, wrist band, smart shoes, clothes,   or earbuds. These gears sense, interact, and transfer data to the receiving devices through Bluetooth 5. Bluetooth 5 works on 2.4GHz band with half/full-duplex mode of transmission and supports IPv6 and AES-128bit security. Moreover, through polling, it provides QoS with a minimum of 3ms latency and 3Mbps of data rate within a 100 meter coverage area. Wi-Fi 6 is one of the booming communication technologies and the integration of Wi-Fi 6 with IoT wearables brings kernel benefits which are not limited to security, interoperability, flexibility, and improvement in data throughput. At the far-edge compute nodes, signaling and sensor data can be analyzed before being transported to the cloud for other analytical tasks. Feedback and insights from analytical tasks can provide vital information to many applications, such as emergency response, medical retrieval, and telecare.

\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/BAN-BLE-Lastest.pdf}
\caption{Communication Scenario for IoT Wearable Applications.}
\label{fig_BAN-BLE}
\end{figure*}

\subsection{Analytics Everywhere for Intelligent Home Applications}

Table \ref{tab:HAN} sketches the significant communication technologies which are appropriate for a medium range coverage. Except for Wi-Fi HaLow and Wireless HART, the majority of them support the IPv6 feature. When designing a medium-range intelligent home application, several types of networks can be considered, including WLAN, LAN, CAN, and HAN \cite{FredericoSensinginSmartHome}. Considering the latency, QoS, power consumption and data rate specification, the preferred technologies for the medium-range IoT system are BLE, Z-wave, Zigbee, and Thread \cite{Domb2019SmartHome}. In terms of wired communication, we can consider ethernet and optical fiber as a backbone for such IoT use cases. WirepasMesh and DigiMesh are both well matched for a mesh network, although, we must consider the fact that the power saving mechanism is not supported by WirepasMesh which is an important disadvantage.

\begin{table*}[!ht]
\centering
\caption{ Communication Technologies suited for Intelligent Home Applications.}
\label{tab:HAN}
\resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
\begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
\midrule
\begin{tabular}[c]{@{}l@{}}BLE (Bluetooth\\ 4/4.1/4.2/5)\end{tabular} & Yes & Half / Full & BAN / WPAN & Yes & 3, 6 & 1, 2, 3 & 0-10 & Yes & 15 - 30, 50 - 70, 100 \\
Bluetooth & No & Half / Full & BAN / WPAN & No & 100 & 1 & 0 - 10 & Yes & 1,10,100 \\
DigiMesh & Yes & Half / Full & WPAN & No & 13 & 0.1152 & 10 - 18 & Yes & 90 - 1600 \\
Ethernet & Yes & Half / Full & LAN / MAN & Yes & 5 - 125 & 1 - 400000 & 40 - 48 & No & 100 \\
Optical Fiber & Yes & Half / Full & LAN / MAN / WAN & Yes & 0.005 & 100 - 43000000 & 30 - 37 & Yes & 550, 1000, 2000, 10000 \\
RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
Thread & Yes & Half & HAN / WPAN & No & 100 & 0.25 & 21 & Yes & 30 \\
Wi-Fi 6 & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & 1.5 & >=1000 & 32 & Yes & 60 - 1000 \\
Wi-Fi  & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & \begin{tabular}[c]{@{}l@{}}1.58, 7.89, 34.87, \\ 58.91, 190 \end{tabular} & \begin{tabular}[c]{@{}l@{}}a/g: 54, b:11, n:600, \\ac:1000, ad:7000, af:568.9, \\ah:347, ax:10000, ay:100000 \end{tabular} & 32 & Yes & 10 - 1000 \\
WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
Wi-Fi HLow & No & Half & CAN / WLAN & Yes & 64 & 0.15 – 4, 0.65 - 7.8 & <30 & Yes & 100 – 1000, 700 \\
Wireless HART & No & Half & CAN / WLAN & Yes & 500 - 1000 & 0.25 & 10 & Yes & 10 - 600 \\
Zigbee & Yes & Half / Full & WPAN & Yes & 20 & 0.02, 0.04, 0.25 & 20 & Yes & 10 - 100 \\
Z-Wave & Yes & Half & WPAN & No & 3000 & 0.0096, 0.04, 0.1 & 0 & Yes & 30, 100 \\
6LoWPAN & Yes & Half & WPAN & Yes & 50 - 250 & 0.25 & 3 - 22 & Yes & 10 - 100 \\\bottomrule
\end{tabular}}
\end{table*}

As an example of a medium-range intelligent home application, Fig. \ref{fig_sim4} illustrates the communication technologies deployed in a HAN combining with the Analytics Everywhere framework to support automated analytical tasks. In intelligent homes as in other IoT use cases, seamless connectivity is an important factor that gives users the flexibility to govern smart sensors from any location \cite{BisioIgorI40SmartHome}. Advanced communication tactics can be used to minimize the power consumption of a smart device and augment its communication efficiency \cite{sovacool2020smart}. Wi-Fi 6, the latest version of Wi-Fi to be rolled out, is providing 1000Mbps of data rate with almost 1.5ms of negligible latency. Moreover, it uses a 6GHz band, which gives less interference compared    to other technologies and provides excellent QoS with  the help of mechanism like hybrid coordination function (HCF) which includes enhanced distributed channel access (for prioritized QoS services), and HCF controlled access (for parameterized QoS services). Federal communication commission (FCC) recently adopted a 6GHz band with new rules for unlicensed spectrum use. 6GHz spectrum has already been used by some licensed services (point-to-point microwave links, fixed satellite systems, etc.) which could increase the chance of harmful interference with unlicensed services (specifically the outdoor operations). FCC permits unlicensed devices to operate at very low-power for indoor operations, and at standard-power with automated frequency control (AFC) mechanism for outdoor operations across the 6GHz band in order to avoid collision with licensed services. The key advantages of Wi-Fi 6 for IoT are TWT, dual carrier modulation (DCM), and the ability to offer lower bandwidth to IoT sensors (a single Resource Unit of 2MHz can be offered to provide 375 Kbps, which is ideal for IoT sensors). This effectively improves the link budget by 8 dB hence improving the range. Wi-Fi 6 is based on orthogonal frequency-division multiple access (OFDMA) allowing simultaneous sessions to transmit together using resource units and trigger frames.  Considering all these facts, Wi-Fi 6 can potentially help in reaching the final goal of intelligent homes, to increase comfort and quality of life for intelligent home residents. In a HAN, accumulated and continuous IoT data streams coming from smart devices can be analyzed at the far-edge and cloud when using an Analytics Everywhere framework. The insights from this process can support robbery detection, energy optimization, and automated gardening.

\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/HAN-Scenario.pdf}
\caption{Communication Scenario for Intelligent Home Applications.}
\label{fig_sim4}
\end{figure*}

\subsection{Analytics Everywhere for IoV Applications}

Table \ref{tab:WAN1} presents different long-range communication technologies that provide MAN/WAN/LPWAN networking. Cellular, Cat-M, Cat-0, and 5G are the principal WAN network, while Weightless W/N/P, LoRaWAN, SigFox, NB-IoT, and EC-GSM-IoT are LPWAN communication technologies. The majority of LPWAN network type serves QoS except LoRaWAN, which is based on slotted alohanet. Most of the LPWAN networks are equipped with better security mechanisms.  NB-IoT is the preference for QoS among LPWAN \cite{MEKKI2019IoV}. LoRaWAN follows a separate network architecture and depending on the sensor node, requires a gateway to communicate with another endpoint, which usually is a star network topology \cite{hyder6lowpanlpwan2016IoV}. LoRaWAN supports 20-65km (dependent on many conditions e.g. spreading factor) of coverage range in a rural area with 13km of stable distance with a 500ms of latency. In contrast, SigFox has a higher latency of 2s in almost 50km of rural coverage area and 11km of stable range. In terms of data rate, LoRaWAN outperforms SigFox. In recent years, Weightless W is one of the rarely used LPWAN communication technologies though it has some advantages like maximum data rate and minimum power ratio among LPWAN protocols. However, LoRaWAN and SigFox seem to own the market in unlicensed spectrum. So, the choice of communication technology relies on the type of IoV applications being used.

\begin{table*}[!ht]
\centering
\caption{Communication Technologies suited for IoV Applications.}
\label{tab:WAN1}
\resizebox{\linewidth}{!}{
\begin{tabular}{llllllllll}
\toprule
\begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
\midrule
Cellular & Yes & Full & MAN / WAN & Yes & 10, 50 & \begin{tabular}[c]{@{}l@{}}1G:0.002, 2G:0.064, \\3G:0.144, 4G:100 - 1000  \end{tabular}& 27, 37 & Yes & 8000 - 40000 \\
Cat-M & No & Half / Full & MAN / WAN & Yes & 10 - 15 & 1 & 23 & Yes & 5000 \\
Cat-0 & No & Half / Full & MAN / WAN & Yes & 18 & 1 & 23 & Yes & 5000 \\
DigiMesh & Yes & Half / Full & WPAN & No & 13 & 0.1152 & 10 - 18 & Yes & 90 - 1600 \\
EC-GSM-IOT & Yes & Half / Full & LPWAN & Yes & 700 - 2000 & 0.24, 0.35 & 23 - 33 & Yes & 15000 \\
LoRaWAN & Yes & Half / Full & LPWAN & Yes & 500 & 0.05, 0.027 & 20 & Yes & 5000, 13000, 20000 \\
NB-IOT & Yes & Half & LPWAN & Yes & <10000 & 0.2, 0.234, 0.2048 & 23 & Yes & 100 - 10000 \\
Optical Fiber & Yes & Half / Full & LAN / MAN / WAN & Yes & 0.005 & 100 - 43000000 & 30 - 37 & Yes & 550, 1000, 2000, 10000 \\
RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
SigFox & Yes & Half & LPWAN & Yes & 2000 & 0.0001, 0.0006 & 21.7 & Yes & 10000, 11000, 50000 \\
WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
WiMAX & Yes & Full & WMAN & Yes & 40 - 60 & 30, 75, 100 & 23 - 43 & Yes & 3500, 10000 \\
Wi-Fi HLow & No & Half & CAN / WLAN & Yes & 64 & 0.15 – 4, 0.65 - 7.8 & <30 & Yes & 100 – 1000, 700 \\
Weightless N & No & Full & LPWAN & No & 8000 - 12000 & 0.03 - 0.1 & 17 & No & 2000 \\
Weightless W & No & Half & LPWAN & Yes & 8000 - 12000 & 0.001 - 10 & 17 & No & 5000 \\
Weightless P & No & Full & LPWAN & Yes & 8000 - 12000 & 0.0002 – 0.1 & 17 & No & 2000 \\
5G & Yes & Full & MAN / WAN & Yes & 1 - 10 & >=1000 & 33 - 43 & Yes & 20000, 45000, 60000 \\\bottomrule
\end{tabular}}
\end{table*}

5G paves the way for IoT with the highest connection density of 1 million devices/km$^2$ compared to other communication technologies \cite{NadeemJavaidIoT5G2018IoV}. That such an immense number of devices could be able to communicate with the Internet within a given space is a gigantic step forward for an application like IoV. Fig. \ref{fig_sim5} illustrates the networking within the context of IoV where far-edge/near-edge/cloud computing continuum can provide plenty of analytical services and applications. In an IoV application, 5G technology plays a pivotal role, since  it provides a special QoS for IoV called V2X QoS. It also provides more than 1000Mbps data rate and supports vehicle telematics, autonomous vehicles, and in-vehicle infotainment applications. In Cellular V2X (C-V2X), it has two interfaces – Uu (long range cellular network communication) and PC5 (short range, network-less, direct communication). The Uu utilizes the 5G spectrum while PC5 is short-range similar to what was supported with DSRC (Dedicated short range communications). V2V, V2I, and V2P communications operating in ITS bands (e.g. 5.9GHz) which is independent of the cellular network whereas V2N communication operates in mobile broadband licensed spectrum.  In this case, the Analytics Everywhere framework is fully utilized by executing multiple analytical capabilities (e.g., descriptive, diagnostic, predictive) on the distributed resources (far-edge/near-edge/cloud continuum) according to a data-life cycle. By combining this framework with an IoV network infrastructure, various applications can be offered such as V2V, V2I, V2H, and V2X (Fig. \ref{fig_sim5}).

\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/IoV-Scenario.pdf}
\caption{Communication Scenario for IoV Applications.}
\label{fig_sim5}
\end{figure*}


% OLD TEXT
%\section{Communication Technologies in Analytics Everywhere for IoT Applications}
% In this section, communication technologies have been compared based on their main specificities.We discuss how they fit into three IoT applications and how their network infrastructure can be integrated into the Analytics Everywhere framework. We demonstrate by describing communication scenarios such as Bluetooth 5, Wi-Fi 6, and 5G, and by sketching three IoT applications: Wearables, Smart Home, and Internet of Vehicles (IoV). 

% \subsection{Analytics Everywhere for Wearable Applications}
% Table \ref{tab:BAN} summarizes the most suitable, stable, and efficient communication technologies available for wearable applications. In a short-range communication scenario (e.g. wireless human sensing, gesture recognition), an RFID solution fits well because of its unique ID. Where, an Wi-Fi-based solution is more useful in the non-intrusive type of human sensing due to its wireless characteristics \cite{LiuZWirelessHumanSensing}, a variety of network types (e.g. BAN, WPAN, and WLAN) can be selected, depending on the requirements of a wearable application. Z-wave has a -20 to 0 dBm power ratio and a sleep/awake power saving mechanism, making it an appropriate match for wearable applications from a network management perspective, since users could manage smart lighting from their smart watches (part of BAN). Z-wave (WPAN) would the give access to a smart hub. Considering energy harvesting and low cost of tags, NFC is crucial for privacy and contactless payments \cite{AntonioNFCsensor}. In terms of coverage range, RF and WirepasMesh can give us the flexibility to go beyond a 100 meter range with IoT wearables. From a security perspective, 6LoWPAN is an exemplary option as it only works with IPv6.

% %Our table would surely help the research community and industry to unearth the most suitable communication technology from this pool of heterogeneous protocols based on specific IoT applications.


% \begin{table*}[!ht]
% \centering
% \caption{Communication Technologies suited for IoT Wearable Applications.}
% \label{tab:BAN}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llllllllll}
% \toprule
% \begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
% \midrule
% ANT & No & Full & WPAN & No & 7.5 - 15 & 1 & \textless 17 & Yes & 30 \\
% \begin{tabular}[c]{@{}l@{}}BLE (Bluetooth\\ 4/4.1/4.2/5)\end{tabular} & Yes & Half / Full & BAN / WPAN & Yes & 3, 6 & 1, 2, 3 & 0 -10 & Yes & 15 - 30, 50 - 70, 100 \\
% Bluetooth & No & Half / Full & BAN / WPAN & No & 100 & 1 & 0 - 10 & Yes & 1,10,100 \\
% EnOcean & Yes & Half & WPAN & No & 40 - 100 & 0.125 & 10 & Yes & 30 \\
% Infrared & Yes & Half & WLAN & Yes & 175 & 12500 & 24 & No & 0.001 - 30 \\
% NFC & Yes & Half & BAN / WPAN & Yes & 125 & \begin{tabular}[c]{@{}l@{}}0.106, 0.212, \\ 0.424, 0.848\end{tabular} & 20, 23 & No & 0.1 - 0.2 \\
% RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
% RFID & Yes & Half / Full & WPAN & Yes & 20 & 0.5 & 1.8 & Yes & 0.1 - 5 \\
% Thread & Yes & Half & HAN / WPAN & No & 100 & 0.25 & 21 & Yes & 30 \\
% WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
% Zigbee & Yes & Half / Full & WPAN & Yes & 20 & 0.02, 0.04, 0.25 & 20 & Yes & 10 - 100 \\
% Z-Wave & Yes & Half & WPAN & No & 3000 & 0.0096, 0.04, 0.1 & -20 - 0 & Yes & 30, 100 \\
% 6LoWPAN & Yes & Half & WPAN & Yes & 50 - 250 & 0.25 & 3 - 22 & Yes & 10 - 100 \\\bottomrule
% \end{tabular}}
% \end{table*}

% Fig. \ref{fig_BAN-BLE} shows a communication scenario for wearable applications operating in BAN where EoG, ECG, and EMG sensors are attached in the form of a small chipset within wearable devices like a smartwatch, wrist band, smart shoes, clothes, or earbuds. These gears sense, interact, and transfer data to the receiving devices through Bluetooth 5. Bluetooth 5 works on 2.4GHz band with half/full-duplex mode of transmission and supports IPv6 and AES-128bit security. Moreover, through polling, it provides QoS with a minimum of 3ms latency and 3Mbps of data rate within a 100 meter coverage area. At the edge compute nodes, signaling and sensor data can be analyzed before being transported to the cloud for other analytical tasks. Feedback and insights from analytical tasks can provide vital information to many applications, such as emergency response, medical retrieval, and telecare.

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=\linewidth]{Figures/BAN-BLE-Lastest.pdf}
% \caption{Communication Scenario for IoT Wearable Applications.}
% \label{fig_BAN-BLE}
% \end{figure*}


% \subsection{Analytics Everywhere for Smart Home Applications}

% Table \ref{tab:HAN} sketches all the communication technologies which are appropriate for a medium range coverage. Except for Wi-Fi HaLow and Wireless HART, the majority of them support the IPv6 feature. When designing a medium-range Smart Home application, several types of networks can be considered, including Wireless Local Area Network (WLAN), Local Area Network (LAN), Campus Area Network (CAN), and Home Area Network (HAN) \cite{FredericoSensinginSmartHome}. Considering the latency, QoS, power consumption and data rate specification, the preferred technologies for the medium-range IoT system are BLE, Z-wave, Zigbee, and Thread \cite{Domb2019SmartHome}. In terms of wired communication, we can consider Ethernet and Optical Fiber as a backbone for such IoT applications. WirepasMesh and DigiMesh are both well matched for a Mesh network, although, we must consider the fact that the power saving mechanism is not supported by WirepasMesh which is an important disadvantage. 

% \begin{table*}[!ht]
% \centering
% \caption{ Communication Technologies suited for Smart Home Applications.}
% \label{tab:HAN}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llllllllll}
% \toprule
% \begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
% \midrule
% \begin{tabular}[c]{@{}l@{}}BLE (Bluetooth\\ 4/4.1/4.2/5)\end{tabular} & Yes & Half / Full & BAN / WPAN & Yes & 3, 6 & 1, 2, 3 & 0-10 & Yes & 15 - 30, 50 - 70, 100 \\
% Bluetooth & No & Half / Full & BAN / WPAN & No & 100 & 1 & 0 - 10 & Yes & 1,10,100 \\
% DigiMesh & Yes & Half / Full & WPAN & No & 13 & 0.1152 & 10 - 18 & Yes & 90 - 1600 \\
% Ethernet & Yes & Half / Full & LAN / MAN & Yes & 5 - 125 & 1 - 400000 & 40 - 48 & No & 100 \\
% Optical Fiber & Yes & Half / Full & LAN / MAN / WAN & Yes & 0.005 & 100 - 43000000 & 30 - 37 & Yes & 550, 1000, 2000, 10000 \\
% RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
% Thread & Yes & Half & HAN / WPAN & No & 100 & 0.25 & 21 & Yes & 30 \\
% Wi-Fi 6 & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & 1.5 & >=1000 & 32 & Yes & 60 - 1000 \\
% Wi-Fi  & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & \begin{tabular}[c]{@{}l@{}}1.58, 7.89, 34.87, \\ 58.91, 190 \end{tabular} & \begin{tabular}[c]{@{}l@{}}a/g: 54, b:11, n:600, \\ac:1000, ad:7000, af:568.9, \\ah:347, ax:10000, ay:100000 \end{tabular} & 32 & Yes & 10 - 1000 \\
% WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
% Wi-Fi HLow & No & Half & CAN / WLAN & Yes & 64 & 0.15 – 4, 0.65 - 7.8 & <30 & Yes & 100 – 1000, 700 \\
% Wireless HART & No & Half & CAN / WLAN & Yes & 500 - 1000 & 0.25 & 10 & Yes & 10 - 600 \\
% Zigbee & Yes & Half / Full & WPAN & Yes & 20 & 0.02, 0.04, 0.25 & 20 & Yes & 10 - 100 \\
% Z-Wave & Yes & Half & WPAN & No & 3000 & 0.0096, 0.04, 0.1 & 0 & Yes & 30, 100 \\
% 6LoWPAN & Yes & Half & WPAN & Yes & 50 - 250 & 0.25 & 3 - 22 & Yes & 10 - 100 \\\bottomrule
% \end{tabular}}
% \end{table*}

% As an example of a medium-range Smart Home application, Fig. \ref{fig_sim4} illustrates the communication technologies deployed in a HAN combining with the Analytics Everywhere framework to support automated analytical tasks. In smart homes as in other IoT applications, seamless connectivity is an important factor that gives users the flexibility to govern smart sensors from any location \cite{BisioIgorI40SmartHome}. Advanced communication tactics can be used to minimize the power consumption of a smart device and augment its communication efficiency \cite{Hory2017SmartHome}. Wi-Fi 6, the latest version of Wi-Fi to be rolled out, is providing 1000Mbps of data rate with almost 1.5ms of negligible latency. Moreover, it uses a 6GHz band, which gives less interference compared to other technologies and provides excellent QoS with the help of several techniques, like contention window and hybrid coordination function. Considering all these facts, Wi-Fi6 can potentially help in reaching the final goal of smart homes, to increase comfort and quality of life for smart home residents. In a HAN, accumulated and continuous IoT data streams coming from smart devices can be analyzed at the edge and cloud when using an Analytics Everywhere framework. The insights from this process can support robbery detection, energy optimization, and automated gardening.   

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=\linewidth]{Figures/HAN-Scenario.pdf}
% \caption{Communication Scenario for Smart Home Applications.}
% \label{fig_sim4}
% \end{figure*}



% \subsection{Analytics Everywhere for IoV Applications}

% Table \ref{tab:WAN1} presents different long-range communication technologies that provide MAN/WAN/LPWAN networking. Cellular, Cat-M, Cat-0, and 5G are the principal WAN network, while Weightless W/N/P, LoRaWAN, SigFox, NB-IoT, and EC-GSM-IoT are LPWAN communication technologies. The majority of LPWAN network type serve QoS and provide better security. NB-IoT is the preference for QoS among LPWAN \cite{MEKKI2019IoV}. LoRaWAN follows a separate network architecture and depending on the sensor node, requires a gateway to communicate with another endpoint, which usually is a star network topology \cite{hyder6lowpanlpwan2016IoV}. LoRaWAN supports 20km of coverage range in a rural area with 13km of stable distance with a 500ms of latency. In contracts, SigFox has a higher latency of 2s in almost 50km of rural coverage area and 11km of stable range. In terms of data rate, LoRaWAN beats SigFox. However, Weightless W has a maximum data rate and minimum power ratio among Low power WAN protocols so, the choice of communication technology relies on the type of IoV applications being used. 

% \begin{table*}[!ht]
% \centering
% \caption{ Communication Technologies suited for IoV Applications.}
% \label{tab:WAN1}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llllllllll}
% \toprule
% \begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
% \midrule
% Cellular & Yes & Full & MAN / WAN & Yes & 10, 50 & \begin{tabular}[c]{@{}l@{}}1G:0.002, 2G:0.064, \\3G:0.144, 4G:100 - 1000  \end{tabular}& 27, 37 & Yes & 8000 - 40000 \\
% Cat-M & No & Half / Full & MAN / WAN & Yes & 10 - 15 & 1 & 23 & Yes & 5000 \\
% Cat-0 & No & Half / Full & MAN / WAN & Yes & 18 & 1 & 23 & Yes & 5000 \\
% DigiMesh & Yes & Half / Full & WPAN & No & 13 & 0.1152 & 10 - 18 & Yes & 90 - 1600 \\
% EC-GSM-IOT & Yes & Half / Full & LPWAN & Yes & 700 - 2000 & 0.24, 0.35 & 23 - 33 & Yes & 15000 \\
% LoRaWAN & Yes & Half / Full & LPWAN & Yes & 500 & 0.05, 0.027 & 20 & Yes & 5000, 13000, 20000 \\
% NB-IOT & Yes & Half & LPWAN & Yes & <10000 & 0.2, 0.234, 0.2048 & 23 & Yes & 100 - 10000 \\
% Optical Fiber & Yes & Half / Full & LAN / MAN / WAN & Yes & 0.005 & 100 - 43000000 & 30 - 37 & Yes & 550, 1000, 2000, 10000 \\
% RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
% SigFox & Yes & Half & LPWAN & Yes & 2000 & 0.0001, 0.0006 & 21.7 & Yes & 10000, 11000, 50000 \\
% WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
% WiMAX & Yes & Full & WMAN & Yes & 40 - 60 & 30, 75, 100 & 23 - 43 & Yes & 3500, 10000 \\
% Wi-Fi HLow & No & Half & CAN / WLAN & Yes & 64 & 0.15 – 4, 0.65 - 7.8 & <30 & Yes & 100 – 1000, 700 \\
% Weightless N & No & Full & LPWAN & No & 8000 - 12000 & 0.03 - 0.1 & 17 & No & 2000 \\
% Weightless W & No & Half & LPWAN & Yes & 8000 - 12000 & 0.001 - 10 & 17 & No & 5000 \\
% Weightless P & No & Full & LPWAN & Yes & 8000 - 12000 & 0.0002 – 0.1 & 17 & No & 2000 \\
% 5G & Yes & Full & MAN / WAN & Yes & 1 - 10 & >=1000 & 33 - 43 & Yes & 20000, 45000, 60000 \\\bottomrule
% \end{tabular}}
% \end{table*}

% %In Table \ref{tab:WAN1}, we have many different MAN/WAN/LPWAN communication technologies apt for IoV.

% 5G paves the way for IoT with the highest connection density of 1 million devices/km$^{2}$ compared to other communication technologies \cite{NadeemJavaidIoT5G2018IoV}. That such an immense number of devices could be able to communicate with the Internet within a given space is a gigantic step forward for an application like IoV. Fig. \ref{fig_sim5} illustrates the networking within the context of IoV where edge/fog/cloud computing continuum can provide plenty of analytical services and applications. In an IoV application, 5G technology plays a pivotal role, since it provides a special QoS for IoV called V2X QoS. It also provides more than 1000Mbps data rate and supports vehicle telematics, autonomous vehicles, and in-vehicle infotainment applications. In this case, the Analytics Everywhere framework is fully utilized by executing multiple analytical capabilities (e.g., descriptive, diagnostic, predictive) on the distributed resources (edge/fog/cloud continuum) according to a data-life cycle. By combining this framework with an IoV network infrastructure, various applications can be offered such as V2V, V2I, V2H, and V2X (Fig. \ref{fig_sim5}).
 

% %In the 5G-IIoT (Intelligent IoT) architecture proposed by Wang D et al, emphasize given to mmWave and massiveMIMO facets of 5G technology which are essential in evolving IoT applications like IoV \cite{DanWang5GIioT2018IoV}. 



% %With the rising numbers of personal and public transportation, vehicular networks have also emerged in IoT. Internet of Vehicles (IoV) is an interconnection to the smart vehicles through vehicular networks. In IoV, Vehicular networks act as a bridge between vehicles and gateway/cloud/other vehicles. 

% %Communication between vehicles is mobile in IoV so they must obligate a long range communication protocol to communicate. %MAN, WAN, and low power WAN are the best-suited types of the network for IoV applications. 

% %In IoV, we should be very concerned about end-user data privacy and security regardless of the type of networks and communication protocols we are using for specific IoV applications to exchange data \cite{juan2018IoV}. 



% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=\linewidth]{Figures/IoV-Scenario.pdf}
% \caption{Communication Scenario for IoV Applications.}
% \label{fig_sim5}
% \end{figure*}

% %IoV makes the navigation of vehicles effortless. 
% %IoV applications have umpteen benefits for various industries like transportation, logistics, and medical sectors. With the help of IoV, we can control the vehicle better, monitor the live traffic in the rural and urban landscape, track of goods in delivery, and have higher chances of reducing accidents. All the advanced technology equipped smart vehicles can send and receive real-time data through various sensors and communication protocols used in vehicular networks. The front/rear camera system in IoV could help us in reporting urgent circumstances to emergency service sectors, with that we could save the lives of many civilians and resolve critical issues briskly \cite{Hasna2019IoV}. 


% % \subsection{Analytics Everywhere for Wearables}

% % The emerging market of the Internet of Things eternally gains rhythm about the opportunities offered by Wearables. Wearable technology and sensors have become part of day-to-day life for most individuals. IoT Wearables are part of Body Area Network (BAN) because sensors in wearables are connected or surrounded by a human or animal body. They also fall into Wireless Personal Area Network (WPAN) and Wireless Local Area Network (WLAN) type of network based on the short distance range of the communication protocols used by wearables. Fig. \ref{fig_BAN-BLE} delineates overall insight of IoT Wearables and its communication in a BAN. Sensors generally attach in the form of a small chipset within the wearable devices like a smartwatch, jewelry, wrist band, smart clothing, sleep mask, biometric insoles, earbuds, and many more. These gears transfer data to the receiving devices through multiple communication protocols, depending on the applications and how it developed. One of the surveys from NASA quoted that they are using smart clothing technology for astronauts to gain access to their milieu, check their health status, and communicate with other astronauts in space. So, this subset of IoT is thriving in the medical and space sector as well. As per the proposed design of a wearable device for tracking FIFA players by Kim H et al., a new version of the BLE is the better option for data transmission as compared to the ultrawideband of the RF as BLE could also cover the entire stadium to track all the athletes. His team performed the accuracy-test using BLE with real soccer players and it showed the splendid outcome \cite{KimHBleTracking}. BLE works on 2.4 GHz band with half/full-duplex mode of transmission and supports IPv6 and AES-128bit security. Moreover, through Bluetooth polling, it provides QOS with a minimum of 3ms latency and 3Mbps of data rate within 100m coverage area. So, BLE is appropriate for a smartwatch and jewelry kind of IoT applications which provide voice assistant feature by Google assistant, Apple Siri, or Amazon Alexa and monitors user-health statistics as well.

% % \begin{figure*}[!ht]
% % \centering
% % \includegraphics[width=\linewidth]{Figures/BAN-BLE.pdf}
% % \caption{Communication Scenario of IoT Wearables}
% % \label{fig_BAN-BLE}
% % \end{figure*}

% % Each communication technology has its essence of the way it communicates and makes transmission of information vigorously depending on the application scenario. In wireless human sensing, for multi-person scenario and gesture recognition, RFID solution fits well because of its unique ID \cite{LiuZWirelessHumanSensing}. Whereas, Wi-Fi-based solutions are more useful in the non-intrusive type of human sensing due to its wireless characteristics \cite{LiuZWirelessHumanSensing}.  Depending on the type of IoT wearables and IoT applications we have a vast variety of BAN, WPAN, and WLAN communication protocols to choose from. With the perspective of network management, Z-wave has 0 dBm power ratio and sleep/awake power saving mechanism so it is an upright match for applications like smart lighting, smart hub, etc. Considering energy harvesting and low cost of tags, NFC is crucial for privacy and contactless payments \cite{AntonioNFCsensor}. In terms of coverage range, RF and WirepasMesh can give us the flexibility to go beyond 100 meters with IoT Wearables. From a security prospect, 6LoWPAN is an exemplary tailor as it only works with IPv6. We compared the several other communication technologies for IoT wearables which portray in table \ref{tab:BAN}, that depicts the latest, stable, and efficient communication technologies for IoT Wearables which essentially require short coverage range to communicate. In this table, we mentioned nine nub characteristics for all wearable communication technologies depending on chief factors like IoT sensors, Communication, Network performance, and Network management. Our table would surely help the research community and industry to unearth the most suitable communication technology from this pool of heterogeneous protocols based on specific IoT applications.

% % \begin{table*}[!ht]
% % \centering
% % \caption{Communication Technologies suited for IoT Wearables in Chronological Manner}
% % \label{tab:BAN}
% % \resizebox{\linewidth}{!}{
% % \begin{tabular}{llllllllll}
% % \toprule
% % \begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
% % \midrule
% % ANT & No & Full & WPAN & No & 7.5 - 15 & 1 & \textless 17 & Yes & 30 \\
% % BLE & Yes & Half / Full & BAN / WPAN & Yes & 3, 6 & 1, 2, 3 & 0 -10 & Yes & 15 - 30, 50 - 70, 100 \\
% % Bluetooth & No & Half / Full & BAN / WPAN & No & 100 & 1 & 0 - 10 & Yes & 1,10,100 \\
% % EnOcean & Yes & Half & WPAN & No & 40 - 100 & 0.125 & 10 & Yes & 30 \\
% % Infrared & Yes & Half & WLAN & Yes & 175 & 12500 & 24 & No & 0.001 - 30 \\
% % NFC & Yes & Half & BAN / WPAN & Yes & 125 & \begin{tabular}[c]{@{}l@{}}0.106, 0.212, \\ 0.424, 0.848\end{tabular} & 20, 23 & No & 0.1 - 0.2 \\
% % RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
% % RFID & Yes & Half / Full & WPAN & Yes & 20 & 0.5 & 1.8 & Yes & 0.1 - 5 \\
% % Thread & Yes & Half & HAN / WPAN & No & 100 & 0.25 & 21 & Yes & 30 \\
% % WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
% % Zigbee & Yes & Half / Full & WPAN & Yes & 20 & 0.02, 0.04, 0.25 & 20 & Yes & 10 - 100 \\
% % Z-Wave & Yes & Half & WPAN & No & 3000 & 0.0096, 0.04, 0.1 & 0 & Yes & 30, 100 \\
% % 6LoWPAN & Yes & Half & WPAN & Yes & 50 - 250 & 0.25 & 3 - 22 & Yes & 10 - 100 \\\bottomrule
% % \end{tabular}}
% % \end{table*}

% % \subsection{Analytics Everywhere for Smart Home}

% % A smart home is another ubiquitous IoT application that requires a medium range of communication, so it falls under Wireless Personal Area Network (WPAN), Wireless Local Area Network (WLAN), Local Area Network (LAN) and Campus Area Network (CAN) type of networks. These network types are based on the coverage range of communication protocols. The assimilation of all the home systems under a single consolidated management system creates the Home Area Network (HAN) \cite{FredericoSensinginSmartHome}.
    
% % Smart lighting, smart meter, home assistant, smart plugs, smart display, thermostat, home security, and smart TV are examples of IoT smart home applications. Smart home technology commonly consists of smart appliances/households, smart hub, gateway, and edge type of sensors, and medium-range communication protocols. On top of that, we can perform data analytics as well, and automation in smart households brought new paths to IoT for managing and combining smart sensors within Smart home. As proposed by Bisio I et al., Smart home is one of the most boosted areas by the revolution of the Industry 4.0 (I4.0) framework for the IoT \cite{BisioIgorI40SmartHome}. Just like other IoT applications, in Smart home, seamless connectivity is a must factor that gives us the flexibility to govern the smart sensors from any corner of the globe.

% % \begin{figure*}[!ht]
% % \centering
% % \includegraphics[width=\linewidth]{Figures/HAN-Scenario.pdf}
% % \caption{Communication Scenario of Smart Home}
% % \label{fig_sim4}
% % \end{figure*}

% % For Smart home, low cost and low power communication technologies are well suited regardless of each communication technology has its advantages and limitations. Advanced communication tactics can be used to minimize the power consumption of the smart device and augment its communication efficiency \cite{Hory2017SmartHome}. Table \ref{tab:HAN} sketches all the communication technologies which are appropriate for the IoT Smart home with respect to parameters like QOS, Data Rate, Power Ratio, Power saving mechanism, etc. Majority of communication protocols used for Smart Home application’s connectivity, support IPv6 feature except for Wi-Fi HaLow and Wireless HART. The preferred protocols for the Smart home system are BLE, Z-wave, Zigbee, and Thread \cite{Domb2019SmartHome}. Hence, the choice of the protocol depends on the type of application and type of use. Wi-Fi 6 is the latest version of Wi-Fi rolling out alongside 5G technology is providing 1000Mbps of data rate with almost 1.5ms of negligible latency. Moreover, it uses now a 6GHz band which gives less interference compared to other technologies and provides excellent QOS with the help of several techniques like contention window and hybrid coordination function. Considering all these facts, Wi-Fi 6 potentially helps Smart home to reach its final goal of giving more comfort and quality of life to end-users. In terms of wired communication, we can consider Ethernet and Optical fiber as a backbone for such IoT applications. WirepasMesh and DigiMesh, both are well matched for a Mesh network. Though, we must consider the fact that the power saving mechanism is not supported by WirepasMesh which is a big disadvantage of it. A variety of communication technologies described in Table \ref{tab:HAN} provide us the comprehensive alternatives for IoT Smart home.

% % \begin{table*}[!ht]
% % \centering
% % \caption{ Communication Technologies suited for Smart Home in Chronological Manner }
% % \label{tab:HAN}
% % \resizebox{\linewidth}{!}{
% % \begin{tabular}{llllllllll}
% % \toprule
% % \begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
% % \midrule
% % BLE & Yes & Half / Full & BAN / WPAN & Yes & 3, 6 & 1, 2, 3 & 0-10 & Yes & 15 - 30, 50 - 70, 100 \\
% % Bluetooth & No & Half / Full & BAN / WPAN & No & 100 & 1 & 0 - 10 & Yes & 1,10,100 \\
% % DigiMesh & Yes & Half / Full & WPAN & No & 13 & 0.1152 & 10 - 18 & Yes & 90 - 1600 \\
% % Ethernet & Yes & Half / Full & LAN / MAN & Yes & 5 - 125 & 1 - 400000 & 40 - 48 & No & 100 \\
% % Optical Fiber & Yes & Half / Full & LAN / MAN / WAN & Yes & 0.005 & 100 - 43000000 & 30 - 37 & Yes & 550, 1000, 2000, 10000 \\
% % RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
% % Thread & Yes & Half & HAN / WPAN & No & 100 & 0.25 & 21 & Yes & 30 \\
% % Wi-Fi 6 & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & 1.5 & >=1000 & 32 & Yes & 60 - 1000 \\
% % Wi-Fi  & Yes & Half & LAN / CAN / WPAN / WLAN & Yes & \begin{tabular}[c]{@{}l@{}}1.58, 7.89, 34.87, \\ 58.91, 190 \end{tabular} & \begin{tabular}[c]{@{}l@{}}a/g: 54, b:11, n:600, \\ac:1000, ad:7000, af:568.9, \\ah:347, ax:10000, ay:100000 \end{tabular} & 32 & Yes & 10 - 1000 \\
% % WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
% % Wi-Fi HLow & No & Half & CAN / WLAN & Yes & 64 & 0.15 – 4, 0.65 - 7.8 & <30 & Yes & 100 – 1000, 700 \\
% % Wireless HART & No & Half & CAN / WLAN & Yes & 500 - 1000 & 0.25 & 10 & Yes & 10 - 600 \\
% % Zigbee & Yes & Half / Full & WPAN & Yes & 20 & 0.02, 0.04, 0.25 & 20 & Yes & 10 - 100 \\
% % Z-Wave & Yes & Half & WPAN & No & 3000 & 0.0096, 0.04, 0.1 & 0 & Yes & 30, 100 \\
% % 6LoWPAN & Yes & Half & WPAN & Yes & 50 - 250 & 0.25 & 3 - 22 & Yes & 10 - 100 \\\bottomrule
% % \end{tabular}}
% % \end{table*}

% % \subsection{Analytics Everywhere for IoV}

% % With the rising numbers of personal and public transportation, vehicular networks have also emerged in IoT. Internet of Vehicles (IoV) is an interconnection to the smart vehicles through vehicular networks. In IoV, Vehicular networks act as a bridge between vehicles and gateway/cloud/other vehicles. Communication between vehicles is mobile in IoV so they must obligate a long range communication protocol to communicate. MAN, WAN, and low power WAN are the best-suited types of the network for IoV applications. In IoV, we should be very concerned about end-user data privacy and security regardless of the type of networks and communication protocols we are using for specific IoV applications to exchange data \cite{juan2018IoV}. The majority of Low power WAN protocols serve QoS and better security. Weightless W/N/P, LoRaWAN, SigFox, NB-IoT, and EC-GSM-IoT are Low power WAN communication technologies. LoRaWAN follows separate network architecture and accordingly to that sensor node requires a gateway to communicate with another endpoint, which fits them in a star network topology \cite{hyder6lowpanlpwan2016IoV}. LoRaWAN supports 20km of coverage range in a rural area with 13km of stable distance and 500ms of latency. Whereas, SigFox has higher latency of 2s in almost 50km of rural coverage area and 11km of stable range. In terms of Data rate, LoRaWAN beats SigFox. Though Weightless W has a maximum data rate and minimum power ratio among Low power WAN protocols so, the choice of communication technology relies on the type of IoV applications. IoT applications, which entail promised QOS, NB-IoT is the finest preference among Low power WAN \cite{MEKKI2019IoV}.

% % \begin{figure*}[!ht]
% % \centering
% % \includegraphics[width=\linewidth]{Figures/IoV-Scenario.pdf}
% % \caption{Communication Scenario of IoV}
% % \label{fig_sim5}
% % \end{figure*}

% % IoV makes the navigation of vehicles effortless. IoV applications have umpteen benefits for various industries like transportation, logistics, and medical sectors. With the help of IoV, we can control the vehicle better, monitor the live traffic in the rural and urban landscape, track of goods in delivery, and have higher chances of reducing accidents. All the advanced technology equipped smart vehicles can send and receive real-time data through various sensors and communication protocols used in vehicular networks. The front/rear camera system in IoV could help us in reporting urgent circumstances to emergency service sectors, with that we could save the lives of many civilians and resolve critical issues briskly \cite{Hasna2019IoV}. In Table \ref{tab:WAN1}, we have many different MAN/WAN/LPWAN communication technologies apt for IoV. Cellular, Cat-M, Cat-0, and 5G are the principal WAN protocols for vehicular networks. Among these WAN protocols, 5G technology paves the way for IoT with the highest connection density of 1 million devices/ km2 compared to other protocols \cite{NadeemJavaidIoT5G2018IoV}. Such an immense number of devices could be able to communicate with the internet within a given space with the help of 5G-IoT is a gigantic step forward for an application like IoV. Moreover, 5G provides special QoS for IoV called V2X QoS which is a vital aspect of IoV applications. In the 5G-IIoT (Intelligent IoT) architecture proposed by Wang D et al, emphasize given to mmWave and massiveMIMO facets of 5G technology which are essential in evolving IoT applications like IoV \cite{DanWang5GIioT2018IoV}. 5G is a more suitable long-range communication technology for IoV as it provides more than 1000Mbps data rate and supports vehicle telematics, autonomous vehicles, and in-vehicle infotainment applications.

% % \begin{table*}[!ht]
% % \centering
% % \caption{ Communication Technologies suited for Internet of Vehicles in Chronological Manner }
% % \label{tab:WAN1}
% % \resizebox{\linewidth}{!}{
% % \begin{tabular}{llllllllll}
% % \toprule
% % \begin{tabular}[c]{@{}l@{}}\textbf{Communication} \\ \textbf{Technologies}\end{tabular} & \textbf{IPv6 Support} & \textbf{Duplex Mode} & \textbf{Type of Network} & \textbf{QoS} & \textbf{Latency (ms)} & \textbf{Data Rate (Mbps)} & \textbf{Power Ratio (dBm)} & \begin{tabular}[c]{@{}l@{}}\textbf{Power} \\ \textbf{Saving} \\ \textbf{Mechanism}\end{tabular} & \textbf{Coverage Range (m)} \\
% % \midrule
% % Cellular & Yes & Full & MAN / WAN & Yes & 10, 50 & \begin{tabular}[c]{@{}l@{}}1G:0.002, 2G:0.064, \\3G:0.144, 4G:100 - 1000  \end{tabular}& 27, 37 & Yes & 8000 - 40000 \\
% % Cat-M & No & Half / Full & MAN / WAN & Yes & 10 - 15 & 1 & 23 & Yes & 5000 \\
% % Cat-0 & No & Half / Full & MAN / WAN & Yes & 18 & 1 & 23 & Yes & 5000 \\
% % DigiMesh & Yes & Half / Full & WPAN & No & 13 & 0.1152 & 10 - 18 & Yes & 90 - 1600 \\
% % EC-GSM-IOT & Yes & Half / Full & LPWAN & Yes & 700 - 2000 & 0.24, 0.35 & 23 - 33 & Yes & 15000 \\
% % LoRaWAN & Yes & Half / Full & LPWAN & Yes & 500 & 0.05, 0.027 & 20 & Yes & 5000, 13000, 20000 \\
% % NB-IOT & Yes & Half & LPWAN & Yes & <10000 & 0.2, 0.234, 0.2048 & 23 & Yes & 100 - 10000 \\
% % Optical Fiber & Yes & Half / Full & LAN / MAN / WAN & Yes & 0.005 & 100 - 43000000 & 30 - 37 & Yes & 550, 1000, 2000, 10000 \\
% % RF & Yes & Half / Full & N/A & Yes & 4.2 & 0.02 - 10000 & 20 - 40 & No & 0.0001 - 100000000 \\
% % SigFox & Yes & Half & LPWAN & Yes & 2000 & 0.0001, 0.0006 & 21.7 & Yes & 10000, 11000, 50000 \\
% % WirepasMesh & Yes & Half / Full & WPAN & Yes & 10 & 1 & 5 & No & 100 - 10000 \\
% % WiMAX & Yes & Full & WMAN & Yes & 40 - 60 & 30, 75, 100 & 23 - 43 & Yes & 3500, 10000 \\
% % Wi-Fi HLow & No & Half & CAN / WLAN & Yes & 64 & 0.15 – 4, 0.65 - 7.8 & <30 & Yes & 100 – 1000, 700 \\
% % Weightless N & No & Full & LPWAN & No & 8000 - 12000 & 0.03 - 0.1 & 17 & No & 2000 \\
% % Weightless W & No & Half & LPWAN & Yes & 8000 - 12000 & 0.001 - 10 & 17 & No & 5000 \\
% % Weightless P & No & Full & LPWAN & Yes & 8000 - 12000 & 0.0002 – 0.1 & 17 & No & 2000 \\
% % 5G & Yes & Full & MAN / WAN & Yes & 1 - 10 & >=1000 & 33 - 43 & Yes & 20000, 45000, 60000 \\\bottomrule
% % \end{tabular}}
% % \end{table*}

